Efficient Subsampled Gauss-Newton and Natural Gradient Methods for Training Neural Networks

We present practical Levenberg-Marquardt variants of Gauss-Newton and natural gradient methods for solving non-convex optimization problems that arise in training deep neural networks involving enormous numbers of variables and huge data sets. Our methods use subsampled Gauss-Newton or Fisher information matrices and either subsampled gradient estimates (fully stochastic) or full gradients (semi-stochastic), which, in the latter case, we prove convergent to a stationary point. By using the Sherman-Morrison-Woodbury formula with automatic differentiation (backpropagation) we show how our methods can be implemented to perform efficiently. Finally, numerical results are presented to demonstrate the effectiveness of our proposed methods.

==> not used/abstract.tex <==
We present practical Levenberg-Marquardt variants of Gauss-Newton and natural gradient methods for solving non-convex optimization problems that arise in training deep neural networks involving enormous numbers of variables and huge data sets. Our methods use subsampled Gauss-Newton or Fisher information matrices and either subsampled gradient estimates (fully stochastic) or full gradients (semi-stochastic), which, in the latter case, we prove convergent to a stationary point. By using the Sherman-Morrison-Woodbury formula with automatic differentiation (backpropagation) we show how our methods can be implemented to perform efficiently. Finally, numerical results are presented to demonstrate the effectiveness of our proposed methods.

==> not used/convergence.tex <==
\section{Convergence}
\label{section_10}


Recall that the LM direction that we compute is
$p_t = - (B_t + \lambda_t I)^{-1} g_t.$
If we let $\Delta_t = ||p_t||$, it is well known that $p_t$ is the global solution to the trust-region (TR) problem
\begin{align*}
    \min_{p} m_t(p) \text{ s.t. } ||p|| \le \Delta_t.
\end{align*}

As in the classical TR method, we evaluate the quality of the quadratic model $m_t(\cdot)$ by computing $\rho_t$ defined by (\ref{equation_24}). However, while the classical TR method updates $\Delta_t$ depending on the value of $\rho_t$, we follow the LM approach of updating $\lambda_t$ instead. Loosely speaking, there is a reciprocal-like relation between $\lambda_t$ and $\Delta_t$. While Martens \cite{martens2010deep} proposed this way of updating $\lambda_t$ as a "heuristic", we are able to show that Algorithm \ref{algo_1}, with a exact (full) gradient (i.e., $N_1 = N$) and only updating $\theta_t$ when $\rho_t$ is above a certain threshold (say $\eta$),
%If $\rho_t > \eta$, $\theta^{(t+1)} = \theta^{(t)} + p_t$; else, $\theta^{(t+1)} = \theta^{(t)}$. {\bf full-grad} option, 
converges to a stationary point under the following assumptions:

%\begin{assumption}
%    $H_i$ is positive semi-definite. (Hence, $B_t$ is positive semi-definite. )
%\end{assumption}

\begin{assumption}
    \label{assumption_5}
    $||B_t|| \le \beta$.
\end{assumption}

\begin{assumption}
    \label{assumption_6}
    $||\nabla^2 f(\theta)|| \le \beta_1$.
\end{assumption}

%\begin{assumption}
%    $f$ is bounded below.
%\end{assumption}

Our proof is similar to that used to prove convergence of the standard trust-region method ( e.g., see \cite{wright1999numerical}), and in particular makes use of the following:
\begin{lemma}
    \label{lemma_1}
    %$m_t(0) - m_t(p_t) \ge c_1 ||g_t|| \min \left( \Delta_t, \frac{||g_t||}{||G_t||} \right)$.
    Under Assumption \ref{assumption_5}, there exists a constant $c_1 > 0$ such that
    $$m_t(0) - m_t(p_t) \ge c_1 ||g_t|| \Delta_t.$$
\end{lemma}

\begin{proof}
Because $p_t = - (B_t + \lambda_t I)^{-1} g_t$, $-g_t^T p_t = p_t^T \left( B_t + \lambda_t I \right) p_t$. Then since $B_t \succeq 0$ , we have
\begin{align*}
    m_t(0) - m_t(p_t)
    & = - g_t^T p_t - \frac{1}{2} p_t^T B_t p_t
%   \\ & = \left( (B_t + \lambda_t I) p_t \right)^T p_t - \frac{1}{2} p_t^T B_t p_t
%   \\ & = p_t^T \left( \frac{1}{2} B_t + \lambda_t I \right) p_t
    %\\ & \ge p_t^T \left( \lambda I \right) p_t
    %\\ & \ge \lambda p_t^T p_t
%   \\
 \ge \lambda_t ||p_t||^2.
\end{align*}
On the other hand, since  $\frac{\lambda_t}{\beta + \lambda_t} \ge \frac{\tau}{\beta + \tau} = c_1 > 0$, $||B_t|| \le \beta$  and $\Delta_t = ||p_t||$,
%(Assumption \ref{assumption_5}),
\begin{align*}
    %c_1 ||g_t|| \min \left( \Delta_t, \frac{||g_t||}{||G_t||} \right)
    c_1 ||g_t|| \Delta_t
    & = c_1 ||- (B_t + \lambda_t I) p_t|| ||p_t||
    %\\ & \le c_1 ||G_t + \lambda I|| ||p_t|| ||p_t||
%    \\ & \le c_1 ||B_t + \lambda_t I|| ||p_t||^2
    %\\ & \le c_1 \left( ||B_t|| + \lambda_t \right) ||p_t||^2
    \le c_1 \left( \beta + \lambda_t \right) ||p_t||^2
%    \\ &
\le \lambda_t ||p_t||^2.
\end{align*}
\end{proof}

Using Lemma \ref{lemma_1}, we now prove the global convergence of the full-gradient variant of Algorithm \ref{algo_1}:
\begin{theorem}
    \label{theorem_3}
    Suppose in Algorithm \ref{algo_1}, we set $N_1 = N$, $\alpha = 1$ and only update $\theta_t$ when $\rho_t \ge \eta$ where $0 < \eta < \epsilon$.
    Then, under Assumptions \ref{assumption_5} and \ref{assumption_6}, if $f$ is bounded below. we have that
    $\lim_{t \to \infty} ||g_t|| = 0.$
\end{theorem}

\begin{proof}

We first show that $\lambda_t$ is bounded above by some constant $\Lambda_1$: Recalling (\ref{equation_24}), at iteration $t$, we have
%\begin{align*}
%    \rho_t = \frac{f(\theta^{(t)}) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)},
%\end{align*}
%and hence,
\begin{align}
    |\rho_t - 1|
    %& = \left| \frac{f(\theta^{(t)}) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} - 1 \right|
    & = \left| \frac{m_t(p_t) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} \right|.
    \label{equation_25}
\end{align}
By Taylor's theorem,
% we have that
%\begin{align*}
$
    f(\theta^{(t)} + p_t) = f(\theta^{(t)}) + \nabla f(\theta^{(t)})^T p_t + \frac{1}{2} p_t^T \nabla^2 f(\theta^{(t)} + \mu p_t) p_t
$
%\end{align*}
for some $\mu \in (0, 1)$. Hence,
\begin{align}
    & \left| m_t(p_t) - f(\theta^{(t)} + p_t) \right|
    %& = \left| f(\theta^{(t)}) + g_t^T p_t + \frac{1}{2} p_t^T G_t p_t - f(\theta^{(t)} + p_t) \right|
    = \left| \frac{1}{2} p_t^T B_t p_t - \frac{1}{2} p_t^T \nabla^2 f(\theta^{(t)} + \mu p_t) p_t \right|
    \le \frac{1}{2} (\beta + \beta_1) ||p_t||^2.
    \label{equation_26}
\end{align}

%On the other hand, because $p_t = - (B_t + \lambda_t I)^{-1} g_t$, we have that
%\begin{align}
%    m_t(0) - m_t(p_t)
%    & = - g_t^T p_t - \frac{1}{2} p_t^T B_t p_t
%    \nonumber
%    \\ & = \left( (B_t + \lambda_t I) p_t \right)^T p_t - \frac{1}{2} p_t^T B_t p_t
%    \nonumber
%    \\ & = p_t^T \left( \frac{1}{2} B_t + \lambda_t I \right) p_t
%    \nonumber
%    %\\ & \ge p_t^T \left( \lambda I \right) p_t
%    %\\ & \ge \lambda p_t^T p_t
%    \\ & \ge \lambda_t ||p_t||^2.
%    \label{equation_27}
%\end{align}

%By Lemma \ref{lemma_1}, we have that for $t \ge T$
%\begin{align}
%    m_t(0) - m_t(p_t) \ge c_1 \epsilon \Delta_t.
%    \label{equation_27}
%\end{align}

By (\ref{equation_25}) and (\ref{equation_26}), we have that
\begin{align*}
    |\rho_t - 1|
    %& = \left| \frac{m_t(p_t) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} \right|
    %\le \frac{\frac{1}{2} (\beta + \beta_1) ||p_t||^2}{c_1 \epsilon \Delta_t}
    \le \frac{\frac{1}{2} (\beta + \beta_1) ||p_t||^2}{\lambda_t ||p_t||^2}
    = \frac{\frac{1}{2} (\beta + \beta_1)}{\lambda_t}.
\end{align*}
%By Assumption \ref{assumption_4},
%\begin{align*}
%    ||p_t||
%    & = ||-(G_t + \lambda_t I)^{-1} g_t||
%    \\ & \le ||(G_t + \lambda_t I)^{-1}|| ||g_t||
%    \\ & \le \frac{\beta_2}{\lambda_t}.
%\end{align*}
%Hence,
%\begin{align*}
%    |\rho_t - 1|
%   & \le \frac{\frac{1}{2} (\beta + \beta_1) \beta_2}{c_1 \epsilon \lambda_t}.
%\end{align*}
Hence, there exists a $\Lambda > 0$ such that for all $\lambda_t \ge \Lambda$, we have $|\rho_t - 1| \le \epsilon$, and thus, $\rho_t \ge 1 - \epsilon$. Consequently, by the way $\lambda_{\text{LM}}$ is updated, for all $t$, $\lambda_t \le boost \cdot                                                                      \Lambda + \tau= \Lambda_1$; i.e.,
 $\lambda_t$ is bounded above. By Assumption \ref{assumption_5}$, ||B_t + \lambda_t I||$ is also bounded, i.e.,  
$
    ||B_t + \lambda_t I||
    %\le ||B_t|| + ||\lambda_t I||
    \le \beta + \Lambda_1
$.
Hence, the minimum eigenvalue of $(B_t + \lambda_t)^{-1}$ is no less than $\frac{1}{\beta + \Lambda_1}$. Finally, by the Cauchy-Schwarz inequality and the fact that $\Delta_t = ||p_t|| = ||-(B_t + \lambda_t I)^{-1} g_t||$, we have that
$
    ||g_t|| \Delta_t
    %\\ = & ||g_t|| ||p_t||
    %\\ = & ||g_t|| ||-(B_t + \lambda_t I)^{-1} g_t||
    \ge ||g_t (B_t + \lambda_t I)^{-1} g_t||
    \ge \frac{1}{\beta + \Lambda_1} ||g_t||^2
$.

Let $T_1 = \{ t = 0,1,... \ | \ \rho_t \ge \eta \}$ denote the set of indices $t$ such that step $p_t$ is accepted. For any $t \in T_1$, by definition of $\rho_t$ and Lemma \ref{lemma_1},
\begin{align}
    f(\theta^{(t)}) - f(\theta^{(t+1)})
    > \eta c_1 ||g_t|| \Delta_t
    \ge \eta c_1  \frac{1}{\beta + \Lambda_1} ||g_t||^2.
    \label{equation_30}
\end{align}

We now show that $|T_1| = \infty$ (unless for some $t$, $g_t = 0$ and Algorithm \ref{algo_1} stops finitely): Suppose
that this is not the case. Then there exists a $T > 0$ such that for all $t \ge T$, $p_t$ is rejected (i.e., $\rho_t \le \eta < \epsilon$). Then, $\lambda_t \to \infty$, contradicting the fact that $\lambda_t$ is bounded. Because $|T_1| = \infty$, $\lim_{t \to \infty} ||g_t|| = \lim_{t \in T_1} ||g_t||$. Because $f$ is bounded below and $f(\theta^{(t)})$ is non-increasing, the left-hand-side of (\ref{equation_30}) goes to zero. Hence, the right-hand-side also goes to zero, which implies $\lim_{t \in T_1} ||g_t|| = 0$. 
\end{proof}

\iffalse

\begin{proof}

First we prove that the following is a 

FALSE STATEMENT: \textit{In Algorithm \ref{algo_1} with full-grad option, if $0 \le \eta \le \frac{1}{4}$, there exists an $\epsilon > 0$ and a positive integer $T > 0$ such that for all $t \ge T$, $||g_t|| \ge \epsilon.$}
    
Suppose, on the contrary, that the statement in the lemma is true. Recalling (\ref{equation_24}), at iteration $t$, we have
%\begin{align*}
%    \rho_t = \frac{f(\theta^{(t)}) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)},
%\end{align*}
%and hence,
\begin{align}
    |\rho_t - 1|
    %& = \left| \frac{f(\theta^{(t)}) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} - 1 \right|
    & = \left| \frac{m_t(p_t) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} \right|.
    \label{equation_25}
\end{align}
By Taylor's theorem,
% we have that
%\begin{align*}
$
    f(\theta^{(t)} + p_t) = f(\theta^{(t)}) + \nabla f(\theta^{(t)})^T p_t + \frac{1}{2} p_t^T \nabla^2 f(\theta^{(t)} + \mu p_t) p_t
$
%\end{align*}
for some $\mu \in (0, 1)$.
Hence,
\begin{align}
    & \left| m_t(p_t) - f(\theta^{(t)} + p_t) \right|
    %& = \left| f(\theta^{(t)}) + g_t^T p_t + \frac{1}{2} p_t^T G_t p_t - f(\theta^{(t)} + p_t) \right|
    \\ = & \left| \frac{1}{2} p_t^T B_t p_t - \frac{1}{2} p_t^T \nabla^2 f(\theta^{(t)} + \mu p_t) p_t \right|
    \nonumber
    \\ \le & \frac{1}{2} (\beta + \beta_1) ||p_t||^2.
    \label{equation_26}
\end{align}

%On the other hand, because $p_t = - (B_t + \lambda_t I)^{-1} g_t$, we have that
%\begin{align}
%    m_t(0) - m_t(p_t)
%    & = - g_t^T p_t - \frac{1}{2} p_t^T B_t p_t
%    \nonumber
%    \\ & = \left( (B_t + \lambda_t I) p_t \right)^T p_t - \frac{1}{2} p_t^T B_t p_t
%    \nonumber
%    \\ & = p_t^T \left( \frac{1}{2} B_t + \lambda_t I \right) p_t
%    \nonumber
%    %\\ & \ge p_t^T \left( \lambda I \right) p_t
%    %\\ & \ge \lambda p_t^T p_t
%    \\ & \ge \lambda_t ||p_t||^2.
%    \label{equation_27}
%\end{align}

%By Lemma \ref{lemma_1}, we have that for $t \ge T$
%\begin{align}
%    m_t(0) - m_t(p_t) \ge c_1 \epsilon \Delta_t.
%    \label{equation_27}
%\end{align}

By (\ref{equation_25}) and (\ref{equation_26}), we have that
\begin{align*}
    |\rho_t - 1|
    %& = \left| \frac{m_t(p_t) - f(\theta^{(t)} + p_t)}{ m_t(0) - m_t(p_t)} \right|
    %\le \frac{\frac{1}{2} (\beta + \beta_1) ||p_t||^2}{c_1 \epsilon \Delta_t}
    \le \frac{\frac{1}{2} (\beta + \beta_1) ||p_t||^2}{\lambda_t ||p_t||^2}
    = \frac{\frac{1}{2} (\beta + \beta_1)}{\lambda_t},
\end{align*}
%By Assumption \ref{assumption_4},
%\begin{align*}
%    ||p_t||
%    & = ||-(G_t + \lambda_t I)^{-1} g_t||
%    \\ & \le ||(G_t + \lambda_t I)^{-1}|| ||g_t||
%    \\ & \le \frac{\beta_2}{\lambda_t}.
%\end{align*}
%Hence,
%\begin{align*}
%    |\rho_t - 1|
%   & \le \frac{\frac{1}{2} (\beta + \beta_1) \beta_2}{c_1 \epsilon \lambda_t}.
%\end{align*}
which implies that there exists a $\Lambda > 0$ such that for all $\lambda_t \ge \Lambda$, we have $|\rho_t - 1| \le \frac{1}{4}$, and thus, $\rho_t \ge \frac{3}{4}$. Consequently, by the way $\lambda_{\text{LM}}$ is updated, for all $t$, $\lambda_t \le \frac{3}{2} \Lambda + \tau$; i.e., $\lambda_t$ is bounded above.
Consider the following two cases:
\begin{enumerate}
    \item There is an infinite sub-sequence $\mathcal{T}$ such that $\rho_t \ge \frac{1}{4}$ for all $t \in \mathcal{T}$:

    Because $0 \le \eta \le \frac{1}{4}$, we accept all steps for $t \in T$, and
     %Thus, for all $t \in \mathcal{T}$, 
     by Lemma \ref{lemma_1},
   % \begin{align*}
   $$
        f(x_t) - f(x_{t+1})
    %    & = f(x_t) - f(x_t + p_t)    \\ & 
        \ge \frac{1}{4} (m_t(0) - m_t(p_t))
    %    \\ & 
    \ge \frac{1}{4}  c_1 \epsilon \Delta_t.
    $$
    %\end{align*}
    Since $f$ is bounded below, we have that
    $\lim_{t \in \mathcal{T}, t \to \infty} \Delta_t = 0.$
    But this is not possible, since, using $\lambda_{\min}(\cdot)$ to denote the smallest eigenvalue of a matrix,
    %\begin{align*}
    $    \Delta_t  = ||p_t|| = ||-(B_t + \lambda_t I)^{-1} g_t||
   %     \\ & = ||(B_t + \lambda_t I)^{-1} \frac{g_t}{||g_t||}|| ||g_t||
   %     \\ & 
   \ge \lambda_{\min} ((B_t + \lambda_t I)^{-1}) \epsilon
    %& \text{($\lambda_{\min}(\cdot)$ denotes the smallest eigenvalue of a matrix)} \\ & 
    \ge (\beta + \frac{3}{2}\Lambda + \tau)^{-1} \epsilon > 0.
    $
   %     \\ & > 0.
   % \end{align*}

    \item There is no such sub-sequence:

    Thus, for sufficient large $t$, $\rho_t < \frac{1}{4}$. By the way $\lambda_{\text{LM}}^{(t)}$ is updated, $\lambda_t \to \infty$, contradicting the fact that
     %by the way $\lambda_{\text{LM}}$ is updated, we have that 
     $\lambda_t$ is bounded above.
\end{enumerate}








%\noindent
%{\bf Proof of Theorem \ref{theorem_3}}

Thus, the statement is false. Now suppose at iteration $m$ that $g_m \neq 0$. Let $\epsilon = \frac{1}{2} ||g_m||$, $R = \frac{\epsilon}{\beta_1}$, and define the ball
%\begin{align*}
$
    B(\theta^{(m)}, R) = \{ \theta | ||\theta - \theta^{(m)} \le R|| \}.
$
%\end{align*}
By Lipschtiz continuity of the gradient, for all $\theta \in B(\theta^{(m)}, R)$,
$
    ||g(\theta)||
    \ge ||g_m|| - ||g_m - g(\theta)||
    \ge 2 \epsilon - \beta_1 ||\theta^{(m)} - \theta||
    \ge \epsilon.
$
%\end{align*}

%We consider two different cases:
%\begin{enumerate}
%    \item $\{ \theta^{(t)} \}_{t \ge m}$ stays inside the ball $B(\theta^{(m)}, R)$:
By the falsity of the statement at the start of the proof, $\{ \theta^{(t)} \}_{t \ge m}$ eventually leaves the ball $B(\theta^{(m)}, R)$:

Let $l \ge m$ denote the first index such that $\theta^{(l+1)} \notin B(\theta^{(m)}, R)$ and $\mathcal{S} = \{ t | m \leq t \leq l, \theta ^{t+1} \neq \theta ^{t} \}$. We have that
    \begin{align*}
        & f(\theta^{(m)}) - f(\theta^{(l+1)})
    %   & = \sum_{t=m}^l f(\theta^{(t)}) - f(\theta^{(t+1)})
    %   \\
        = \sum_{t \in \mathcal{S} } f(\theta^{(t)}) - f(\theta^{(t+1)})
        \\ \ge & \sum_{t \in \mathcal{S} } \eta \left( m_t(0) - m_t(p_t) \right)
        \ge \sum_{t \in \mathcal{S} } \eta c_1 ||g_t|| \Delta_t
        \\ \ge & \sum_{t \in \mathcal{S} } \eta c_1 \epsilon ||p_t||
        %\\ & = \eta c_1 \epsilon \sum_{m \le t \le l, \theta^{(t)} \neq \theta^{(t+1)}} \Delta_t
        %\\ & = \eta c_1 \epsilon \sum_{m \le t \le l, \theta^{(t)} \neq \theta^{(t+1)}} ||p_t||
        \ge \eta c_1 \epsilon R
        = \eta c_1 \frac{\epsilon^2}{\beta_1}.
    \end{align*}
%\end{enumerate}

Because $\{ f(\theta^{(t)}) \}_{t=0}^{\infty}$ is decreasing, there exists a $f^* > - \infty$ such that
%\begin{align*}
$
    \lim_{t \to \infty} f(\theta^{(t)}) = f^*.
$
%\end{align*}
Hence,
%\begin{align*}
$   f(\theta^{(m)}) - f^*
    \ge f(\theta^{(m)}) - f(\theta^{(l+1)})
 \ge \eta c_1 \epsilon^2 \frac{1}{\beta_1}
 \ge \frac{1}{4} \eta c_1 ||g_m||^2 \frac{1}{\beta_1}.
 $
%\end{align*}
Since $f(\theta^{(m)}) - f^* \to 0$, we have that $g_m \to 0$.


\end{proof}
\fi

==> not used/introduction.tex <==
\section{Introduction}

First-order stochastic methods are predominantly used to train deep neural networks (NN), including mini-batch gradient descent (SGD) and its variants that use momentum and acceleration \cite{bottou2018optimization, qian1999momentum} and an adaptive learning rate \cite{duchi2011adaptive, kingma2014adam}. 
%Momentum \cite{qian1999momentum} reduces the oscillatory (noisy) nature of stochastic gradients by adding a multiple of the previous step as a momentum term to the current update. 
First-order methods are easy to implement, and only require moderate computational cost per iteration. However, it is cumbersome to tune their hyper-parameters (e.g., learning rate), and they are often slow to escape from regions where the objective function's Hessian matrix is ill-conditioned. Although adaptive learning rate methods converge fast on the training set, pure SGD is still of interest as it sometimes has better generalization property (\cite{keskar2017improving}).

Second-order stochastic methods have also been proposed for training deep NNs because they take far fewer iterations to converge to a solution by using knowledge of the curvature of the objective function. They also have the ability to both escape from regions where the Hessian of objective function is ill-conditioned, and provide adaptive learning rates. Their main drawback is that, due to the huge number of parameters that deep NNs have, it is practically impossible to compute and invert a full Hessian matrix. Efforts to overcome this problem include Hessian-free inexact Newton methods, stochastic L-BFGS methods, Gauss-Newton and natural gradient methods and diagonal scaling methods. See \cite{bottou2018optimization} for a review of these approaches and relevant references.

\subsection{Our Contributions}

Our main contribution is the development of methods for training deep NNs that incorporate partial, but substantial, second-order information, while keeping the computational cost of each iteration comparable to that required by first-order methods. To achieve this, we propose new generic subsampled generalized Gauss-Newton and natural gradient methods that can be implemented efficiently and are provably convergent. Our methods add a Levenberg-Marquardt (LM) damping term to  the Gauss-Newton and Fisher information matrices and invert the resulting matrices using the Sherman-Morrison-Woodbury formula. Moreover, by taking advantage of the Kronecker factored structure in these matrices, we are able to form and invert them in $O(n)$ time. Furthermore, we prove that semi-stochastic versions of our algorithms (i.e., those that use a full gradient combined with mini-batch stochastic Gauss-Newton or Fisher information matrices) converge to a stationary point. 
%{\bf (need to discuss) By combining momentum and adaptive learning rate approaches that have been used to accelerate stochastic gradient descent with our Newton-like directions, we are able to achieve comparable performance to the state-of-the-art algorithms such as Adam.} 
We demonstrate the effectiveness of our methods with numerical experiment, comparing both first-order method (SGD) and second-order methods (Hessian-free, KFAC). 

%To summarize, our algorithms: 

%\vskip -0.08in
%1. efficiently compute both exact and inexact LevenbergMarquardt modified Gauss-Newton steps; 

%\vskip -0.08in
%2. have provable convergence guarantees; 

%\vskip -0.08in
%3. have stochastic variants that perform competitively. 



\subsection{Closely Related Work}

Our methods were initially motivated by the Hessian-free approach of \cite{martens2010deep}, which approximates the Hessian by the generalized Gauss-Newton matrix and then approximately solves the huge $n \times n$ linear system involving that matrix and an LM damping term to update the $n$ parameters of the NN by an ”early-termination” linear CG method. Other closely related methods include the Krylov subspace descent method of \cite{vinyals2012krylov}, which generalizes the Hessian-free approach by constructing a Krylov subspace; the KFAC method \cite{martens2015optimizing}, which uses the block-diagonal part of the Fisher matrix to approximate the Hessian; and the Kronecker Factored Recursive Approximation method \cite{botev2017practical}, which uses a block-diagonal approximation of the Gauss-Newton matrix. 
%There are also several papers focusing on natural gradient method with generalized inverse of Fisher matrix \cite{bernacchia2018exact, cai2019gram, zhang2019fast}. 
For very recent work  on properties of the natural gradient method and the Fisher matrix in the context of NNs see \cite{bernacchia2018exact, cai2019gram, zhang2019fast}. 



%\cite{kunstner2019limitations}



%In this paper we concentrate on the Hessian-free approach of \cite{martens2010deep}, which approximates the Hessian by the generalized Gauss-Newton matrix and then approximately solves the linear system involving that matrix to update the NN parameters by an "early-termination" linear conjugate gradient method. Other closely related methods include the Krylov subspace descent method of \cite{vinyals2012krylov}, which generalizes the Hessian-free approach by constructing a Krylov subspace; the K-FAC method \cite{martens2015optimizing}, which uses the block-diagonal part of the Fisher matrix to approximate the Hessian; and the Kronecker Factored Recursive Approximation method \cite{botev2017practical}, which uses a block-diagonal approximation of the Gauss-Newton matrix.

==> not used/numerical_experiments.tex <==
\section{Numerical Experiments}

\label{section_17}



\begin{figure}[h]
    % \centering
    \hspace*{-1.6cm}\includegraphics[width = 1.25 \textwidth]{figures/2019-5-22-20-33-56-MNIST-classification.pdf}
    \caption{Results on MNIST classification problem with $N_1 = 60$, $N_2 = 30$. Learning rates: 0.1}
    \label{figure_6}
\end{figure}

\begin{figure}[h]
    \hspace*{-1.6cm}\includegraphics[width= 1.25 \textwidth]{figures/2019-5-22-20-34-46-CIFAR.pdf}
    \caption{Results on CIFAR classification problem with $N_1 = 100$, $N_2 = 50$. Learning rates: 0.01}
    \label{figure_7}
\end{figure}

\begin{figure}[h]
    \hspace*{-1.6cm}\includegraphics[width= 1.25 \textwidth]{figures/2019-5-22-23-48-35-webspam.pdf}
    \caption{Results on webspam classification problem with $N_1 = 60$, $N_2 = 30$. Learning rates: 0.4 (SGD), 0.05 (HF and SMW-GN), 0.1 (SMW-NG, SMW-NG and KFAC)}
    \label{figure_8}
\end{figure}

We compared our algorithms SMW-GN and SMW-NG with SGD, HF and KFAC. The KFAC algorithm was implemented using block-diagonal approximaton, without re-scaling and momentum (see section 6.4 and 7 of \cite{martens2015optimizing}). We also included a block diagonal version of SMW-NG, namely, SMW-NG-BD, where in each block, the matrix is inverted by SMW, in order to mimic the block diagonal approximation used by KFAC. 

For all of the experiments reported in this section, we set the initial value of $\lambda_{\text{LM}}$ to be 1, $boost = 1.01$, $drop = 0.99$, $\epsilon = 1/4$, $\tau = 0.001$, same as in \cite{kiros2013training}.
%and we chose an initialize parameter vector $\theta$ using the random sparse scheme proposed in Section 5 of \cite{martens2010deep}. 
%We used Algorithm \ref{algo_1} with the {\bf stoch-grad} option in all of the numerical experiments reported in this section, because computing full gradients in training neural networks is too expensive. 
All algorithms were implemented in MATLAB R2019a and run on an Intel Core i5 processor.
%Table \ref{table_4} summarizes the data sets that we used in our experiments. 
%Experiments on Algorithm \ref{algo_1} with the {\bf full-grad} option are presented in the supplementary material. 
%We primarily present numerical results regarding the quality of stochastic gradient and stochastic LM directions and how efficiently we can compute them. 
%More sophisticated results including adding adaptive learning rate (Adam \cite{kingma2014adam}) on top of them is included in the supplementary material, showing that our GN/NG methods are compatible with such modification. 
We tested the performance of the algorithms on several classification problems. We reported both training loss and testing error. The data sets were scaled to have zero means and unit variances.


    

%\begin{minipage}{15cm}

%\begin{enumerate}
    %\item 
    {\bf MNIST} (\cite{lecun1998gradient}):
%\label{section_13}
    %We tested the performance of various algorithms on the problem of classifying MNIST. 
    The training set is of size $N = 6 \times 10^4$. We used a NN with one hidden layer of size 500 and logistic activation, i.e., $(m_0, m_1, m_2) = (784, 500, 10)$, where the first and last layers are the size of input and output. The output layer was softmax with cross entropy.  The learning rate for SGD was set to be 0.1, tuned from $\{ 0.01, 0.05, 0.1, 0.5 \}$. Initial learning rates for other methods were also set to be 0.1 for purposes of comparison. We did not tune the learning rates for second-order methods because they adaptively modify the rate by updating $\lambda_{\text{LM}}$ as they proceed. We ran each algorithm for 10 epochs. The results are presented in Figure \ref{figure_6}.


%SGD best learning rate: 0.1, chosen from $[0.01, 0.05, 0.1, 0.5]$. Learning rate is set to be 0.1 for all methods. 

% fully-connected network

% relu / logistic
    
    %\item 
    {\bf CIFAR-10} (\cite{krizhevsky2009learning}):
    %We also tested the performance of various algorithms on the problem of classifying CIFAR-10 . 
    The training set is of size $N = 5 \times 10^4$. We used a NN with two hidden layers of size 400 and logistic activation, i.e., $(m_0, m_1, m_2, m_3) = (3072, 400, 400, 10)$. The output layer was softmax with cross entropy. The learning rate was set to be 0.01. We ran each algorithm for 10 epochs. The results are presented in Figure \ref{figure_7}.
%From Figure \ref{figure_6}, we can see that the performance exhibited by both SMW-CG-explicit and SMW-explicit is consistently competitive with Adam. 


    
    %\item 
    {\bf webspam} (\cite{CC01a}):
    %We also tested the performance of various algorithms on the problem of classifying webspam . 
    The training set is of size $N = 3 \times 10^5$. We used a NN with two hidden layers of size 400 and logistic activation, i.e., $(m_0, m_1, m_2, m_3) = (254, 400, 400, 1)$. Because this is a binary classification, we set the output layer to be logistic with binary cross entropy. 
    %The learning rate was set to be 0.01. 
    We tuned the learning rate for SGD and initial learning rates for other algorithms separately, and the results shown in Figure \ref{figure_8} all used their corresponding best learning rates, which are indicated there.
    We ran each algorithm for 1 epoch. 
    %The results are presented in Figure \ref{figure_8}.
    
%\end{enumerate}
%\end{minipage}









\iffalse
\begin{table}[t]
%\caption{Data sets used}
%\label{table_3}
\caption{Datasets}
\label{table_4}
\vskip 0.1in
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{lccr}
%\toprule
\hline
Name & \# data points $N$ & Input Size $m_0$ & Problem \\
%\midrule
\hline
a1a & 30000 (rounded) & 123 & binary \\
MNIST & 60000 & $28 \times 28$ \\
CURVES & 20000 & $28 \times 28$ \\
webspam & 350000 & 254 & binary \\
USPS & 7200 (rounded) & & Multi-class \\
australian & 600 (rounded) & & binary \\
CIFAR-10 & 50000 \\
%\bottomrule
\hline
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in

\end{table}
\fi

%For all of our algorithms that used the linear conjugate method to solve (\ref{equation_29}) for $q_t$ we used the same early termination approach of \cite{martens2010deep}, i.e., terminating once the relative per-iteration progress made in minimizing a relevant quadratic function falls below some tolerance.

\subsection{Discussion of results}

%\begin{enumerate}

%\item HF
Interestingly, the relative ranking of the algorithms changes from one problem to another, indicating that the relative performance of the algorithms depends upon the data set, structure of the NN, and parameter settings. 
%Both SMW-GN and SMW-Fisher provide useful alternatives to the off-the-shelf algorithms and show decent performance. 

From our experimental results, we see that SMW-GN is always faster than HF in terms of both epochs and clock-time, which is consistent with our analysis above. 
%\item KFAC
KFAC sometimes performs very well, not surprisingly, because it accumulates more and more curvature information with each new mini-batch. But it also slows down considerably when the NN has wide layers (see Figure \ref{figure_7}).  
%\item SGD
Moreover, the three experiments were done differently, mimicing the different practices used when training a NN model, namely, tuning learning rates for all algorithms, tuning learning rates for one algorithm and then using it for all, or simply choosing a conservative learning rate.
After carefully tuning the learning rate, SGD can perform as well as second-order methods as shown in Figure \ref{figure_6}. However, if learning rate is chosen to be more conservative or typical (e.g., 0.01), it may suffer from slow convergence compared with second-order methods (see Figure \ref{figure_7}). If we want to get lower training loss or testing error, we may have to run it for far more epochs / time. 



The key take-away from our numerical results is that our SMW-based algorithms that are based on the Gauss-Newton and natural 
gradient methods are competitive with their Hessian-free and Kronecker-factor implementations, HF and KFAC, as well as SGD. In particular, SMW-GN performs extremely well without requiring any parameter tuning.



%\end{enumerate}












% CNN / fully connected

%\subsection{Experiment 4: Auto-encoder on MNIST}







%\subsection{Comparison between with/without an Adam-like momentum term}

%While a plain momentum-based method updates all parameters with the same learning rate, adaptive learning rate methods \cite{duchi2011adaptive} set the individual learning rates for every parameter based on a second-order component-wise estimate to the gradient. Different versions of these techniques result in sophisticated algorithms such as Adadelta \cite{zeiler2012adadelta}, RMSprop\cite{tieleman2012lecture}, and Adam \cite{kingma2014adam}. \cite{ruder2016overview} offers a good overview of various first-order methods for training neural networks.

%\subsection{hyper-parameter search}

%\subsubsection{$N_1$, $N_2$}

%$$\text{below: ICML version}$$

%\begin{figure*}[hbt]
    %\centering
%    \begin{minipage}[t]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{figures/figure9.eps}
%    \end{minipage}
%    \begin{minipage}[t]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{figures/figure19.eps}
%    \end{minipage}
%    \begin{minipage}[t]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{figures/figure16.eps}
%    \end{minipage}
%    \begin{minipage}[t]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{figures/figure20.eps}
%    \end{minipage}
%    \caption{Results on a1a (left) and webspam (right) binary classification problems with stochastic gradients}
%    \label{figure_3}
%\end{figure*}



\iffalse
\begin{table}[t]
\caption{Data sets used}
\label{table_3}
\vskip 0.1in
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{lcccr}
%\toprule
\hline
Name & \# data points $N$ & Input Size $m_0$ \\
%\midrule
\hline
a1a & 30000 (rounded) & 123 \\
MNIST & 60000 & $28 \times 28$ \\
CURVES & 20000 & $28 \times 28$ \\
webspam & 350000 & 254 \\
%\bottomrule
\hline
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
\fi

%\begin{enumerate}
    %\item a1a\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/binary.html}}:

    %30000 training, 1600 test (truncated).

    %\item MNIST\footnote{\url{http://yann.lecun.com/exdb/mnist/}}:

    %The MNIST dataset was used in both Martens 2010 and Hinton 2006.
    %The MNIST data set consisits of $28 \times 28$ images of hand-written digits. There are 60000 training samples and 10000 testing samples.

    %\item CURVES:

    %20000 training, 10000 testing. $28 \times 28$ images.

    %\item webspam\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/binary.html}}:

    %350,000 samples. 254 features.
%\end{enumerate}








\iffalse
\subsection{Binary Classification}

We tested the performance of Algorithm \ref{algo_1} with {\bf stoch-grad} option on binary classification problems with two data sets, namely, a1a and webspam. The size of the layers are
$(m_1, m_2, m_3) = (500, 300, 1).$
The nonlinear function on each layer is logistic. The loss function is entropy loss. We set $N_1 = 30$, $N_2 = 15$. 

As shown in Figures \ref{figure_3} (first two: a1a, last two: webspam), both SMW-CG-explicit and SMW-explict achieve results that are comparable results to those achieved by Adam in terms of time. In terms of descent per iteration, all stochastic LM methods descend faster than Adam. When compared with KFAC, KFAC descents faster than both Adam and our algorithms on the a1a dataset, while, it goes to a worse stationary point on the webspam data set. 
\fi
